AGATHA: Automatic Graph-mining And Transformer based Hypothesis generation Approach

Medical research is risky and expensive. Drug discovery, as an example, requires that researchers efficiently winnow thousands of potential targets to a small candidate set for more thorough evaluation. However, research groups spend significant time and money to perform the experiments necessary to determine this candidate set long before seeing intermediate results. Hypothesis generation systems address this challenge by mining the wealth of publicly available scientific information to predict plausible research directions. We present AGATHA, a deep-learning hypothesis generation system that can introduce data-driven insights earlier in the discovery process. Through a learned ranking criteria, this system quickly prioritizes plausible term-pairs among entity sets, allowing us to recommend new research directions. We massively validate our system with a temporal holdout wherein we predict connections first introduced after 2015 using data published beforehand. We additionally explore biomedical sub-domains, and demonstrate AGATHA's predictive capacity across the twenty most popular relationship types. This system achieves best-in-class performance on an established benchmark, and demonstrates high recommendation scores across subdomains. Reproducibility: All code, experimental data, and pre-trained models are available online: sybrandt.com/2020/agatha

==> preface.tex <==
% This section allows us to modify preloaded package properties
\makeatletter
% These magic runes make comment's appear inline
% These also need to be above the other magic runes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{regexpatch}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}

% These magic runes make the new changes package work with comments
\usepackage{comment}
\let\wfs@comment@comment\comment
\let\comment\@undefined
\usepackage{changes}
\let\wfs@changes@comment\comment
\let\comment\@undefined
\newcommand\comment{%
    \ifthenelse{\equal{\@currenvir}{comment}}
    {\wfs@comment@comment}
    {\wfs@changes@comment}%
}
\makeatother

% Typical preloader time

\usepackage{hyperref}
\usepackage{multirow}
\usepackage{outlines}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{float}
\usepackage{nicefrac}
\usepackage{url}
\usepackage{booktabs}

% Changes Authors
\definechangesauthor[name="Justin Sybrandt", color=blue]{js}
\definechangesauthor[name="Ilya Tyagin", color=green]{it}
\definechangesauthor[name="Ilya Safro", color=red]{is}


\newcommand{\pymoliererepo}{
\href{http://sybrandt.com/2020/agatha}
{sybrandt.com/2020/agatha}
}
\newcommand{\pymoliere}{AGATHA}

% These are shortcuts for leaving specific changes comments
\newcommand{\note}[2]{\added[id=#1, comment={#2}]{}}

% Justin's add, delete, replace
\newcommand{\Ajs}[1]{\added[id=js]{#1}}
\newcommand{\Djs}[1]{\deleted[id=js]{#1}}
\newcommand{\Rjs}[2]{\replaced[id=js]{#1}{#2}}

% ITyagin's add, delete replace
\newcommand{\Ait}[1]{\added[id=it]{#1}}
\newcommand{\Dit}[1]{\deleted[id=it]{#1}}
\newcommand{\Rit}[2]{\replaced[id=it]{#1}{#2}}

% ISafro's add, delete, replace
\newcommand{\Ais}[1]{\added[id=is]{#1}}
\newcommand{\Dis}[1]{\deleted[id=is]{#1}}
\newcommand{\Ris}[2]{\replaced[id=is]{#1}{#2}}

% THIS ALLOWS FOR CONDITIONAL COMMENTS
\newif\ifthesis
% Comment/ un-comment as needed
\thesisfalse
%\thesistrue

% THIS ALLOWS FOR CONDITIONAL COMMENTS
\newif\ifarxiv
% Comment/ un-comment as needed
\arxivfalse
%\arxivtrue

% Comment out a block of text for KDD (but keep for thesis) with this syntax:
% \ifthesis
% <Text to comment out>
% \else [Optional]
% <Optional replacement for KDD Version>
% \fi

\hyphenation{
    AG-A-THA
}

% These magic runes make everything denser
\setlength{\textfloatsep}{3pt}
\setlength{\floatsep}{3pt}
\setlength{\belowdisplayskip}{3pt} \setlength{\belowdisplayshortskip}{3pt}
\setlength{\abovedisplayskip}{3pt} \setlength{\abovedisplayshortskip}{3pt}



==> tables/pymoliere_256_per_type.tex <==
\begin{table*}
\begin{tabular}{lrrrrrrrrrrr}
\toprule
         Type &   PR &  ROC &   RR &  P@10 &  P@100 &  AP@10 &  AP@100 &  MAP@10 &  MAP@100 &  MRR@10 &  MRR@100 \\
\midrule
 (gngm, celf) & 0.35 & 0.54 & 1.00 &  0.40 &   0.30 &   0.71 &    0.37 &    0.49 &     0.49 &    0.52 &     0.52 \\
 (gngm, neop) & 0.28 & 0.57 & 1.00 &  0.50 &   0.24 &   0.72 &    0.40 &    0.38 &     0.35 &    0.42 &     0.42 \\
 (aapp, neop) & 0.19 & 0.61 & 0.20 &  0.20 &   0.18 &   0.21 &    0.25 &    0.37 &     0.33 &    0.42 &     0.43 \\
 (gngm, cell) & 0.18 & 0.68 & 1.00 &  0.30 &   0.23 &   0.51 &    0.33 &    0.36 &     0.32 &    0.39 &     0.40 \\
 (aapp, cell) & 0.17 & 0.59 & 0.50 &  0.40 &   0.19 &   0.37 &    0.27 &    0.33 &     0.31 &    0.36 &     0.36 \\
 (cell, aapp) & 0.17 & 0.65 & 1.00 &  0.30 &   0.22 &   0.63 &    0.29 &    0.35 &     0.30 &    0.40 &     0.41 \\
 (aapp, gngm) & 0.15 & 0.65 & 0.50 &  0.40 &   0.13 &   0.54 &    0.28 &    0.31 &     0.25 &    0.35 &     0.36 \\
 (gngm, gngm) & 0.15 & 0.62 & 0.50 &  0.10 &   0.18 &   0.50 &    0.19 &    0.31 &     0.25 &    0.34 &     0.35 \\
 (aapp, dsyn) & 0.14 & 0.67 & 0.50 &  0.20 &   0.22 &   0.36 &    0.24 &    0.31 &     0.26 &    0.35 &     0.36 \\
 (bpoc, aapp) & 0.13 & 0.66 & 0.08 &  0.00 &   0.16 &   0.00 &    0.20 &    0.32 &     0.28 &    0.35 &     0.36 \\
 (gngm, dsyn) & 0.13 & 0.68 & 1.00 &  0.40 &   0.20 &   0.62 &    0.35 &    0.25 &     0.21 &    0.28 &     0.29 \\
 (orch, gngm) & 0.13 & 0.65 & 0.50 &  0.10 &   0.12 &   0.50 &    0.14 &    0.26 &     0.23 &    0.29 &     0.31 \\
 (bacs, gngm) & 0.11 & 0.67 & 0.09 &  0.00 &   0.10 &   0.00 &    0.08 &    0.24 &     0.23 &    0.26 &     0.27 \\
 (bacs, aapp) & 0.10 & 0.67 & 0.09 &  0.00 &   0.12 &   0.00 &    0.13 &    0.24 &     0.24 &    0.25 &     0.27 \\
 (aapp, aapp) & 0.09 & 0.68 & 0.08 &  0.00 &   0.11 &   0.00 &    0.10 &    0.24 &     0.20 &    0.26 &     0.28 \\
 (dsyn, humn) & 0.09 & 0.57 & 0.17 &  0.10 &   0.10 &   0.17 &    0.12 &    0.25 &     0.21 &    0.29 &     0.31 \\
 (gngm, aapp) & 0.09 & 0.67 & 0.06 &  0.00 &   0.11 &   0.00 &    0.13 &    0.23 &     0.19 &    0.26 &     0.27 \\
 (phsu, dsyn) & 0.09 & 0.59 & 0.14 &  0.10 &   0.06 &   0.14 &    0.09 &    0.24 &     0.20 &    0.25 &     0.27 \\
 (dsyn, dsyn) & 0.08 & 0.60 & 0.06 &  0.00 &   0.10 &   0.00 &    0.10 &    0.21 &     0.16 &    0.23 &     0.24 \\
 (topp, dsyn) & 0.08 & 0.58 & 1.00 &  0.20 &   0.15 &   0.61 &    0.23 &    0.27 &     0.20 &    0.29 &     0.31 \\
\bottomrule
\end{tabular}
\caption{\pymoliere-256}
\label{tab:pymoliere_256}
\end{table*}
